Identifying Effects of Multivalued Treatments

Multivalued treatment models have typically been studied under restrictive assumptions: ordered choice, and more recently unordered monotonicity. We show how treatment effects can be identified in a more general class of models that allows for multidimensional unobserved heterogeneity. Our results rely on two main assumptions: treatment assignment must be a measurable function of threshold-crossing rules, and enough continuous instruments must be available. We illustrate our approach for several classes of models.

==> mynewmacs.tex <==
% comment out
\newcommand{\commentbs}[1]{}

% absolute value, and norm
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\norm}[1]{\lVert#1\rVert}

% dot product with <..,...> brackets
\newcommand{\bdot}[2]{\langle  #1,#2 \rangle}

% average for i=1 to n:
\newcommand{\avein}{\frac{1}{n}\sum_{i=1}^n}
% sum for i=1 to n:
\newcommand{\sumin}{\sum_{i=1}^n}

%
%                Pour Prosper:
%
\newcommand{\bslpp}[1]{\begin{slide}[Wipe]{{\small #1}}}
\newcommand{\eslpp}{\end{slide}}
\newcommand{\bitst}{\begin{itemstep}
         \item[]
         \vspace{-4mm}
}
\newcommand{\eitst}{\end{itemstep}}
%
%
%        \revbar{texte} writes texte in a paragraph with a revision bar
%
\def\revbar#1{\smallskip \hbox{\hskip -4pt\vrule\hskip 4pt\vbox{#1}}}
%
%         i circonflexe
%
\def\ii{\^{\i}}
%
%         inline fractions of the 1/2 type
%
\def\tfrac#1/#2{\leavevmode
        \kern.1em \raise .5ex \hbox{\the\scriptfont0 #1}%
        \kern-.1em $/$%
        \kern-.15em \lower .25ex \hbox{\the\scriptfont0 #2}}
%
%        \obeywhitespace: print whitespace as seen (except for tabs)
%
\def\makeactive#1{\catcode`#1=\active \ignorespaces}
\def\alwaysspace{\hglue\fontdimen2\the\font \relax}%
{\makeactive\^^M \makeactive\ %
\gdef\obeywhitespace{%
\makeactive\^^M\def^^M{\par\indent}%
\makeactive\ \let =\alwaysspace}}%
%
%          IN MATH MODE:
%
%               overline/underline
%
\newcommand{\ov}[1]{\overline{#1}}
\newcommand{\uv}[1]{\underline{#1}}
%
%     partial derivatives
%
\newcommand{\dpart}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\ddpart}[3]{\frac{\partial^2 #1}{\partial #2 \partial #3}}
\newcommand{\ddeux}[2]{\frac{\partial^2 #1}{\partial {#2}^{2}}}
\newcommand{\ddpartd}[2]{\frac{\partial^2 #1}{\partial #2^{2}}}
%
%     the real etc lines
%
\def\bkR{{\rm I\kern-.17em R}}
\def\bkQ{{\rm I\kern-.17em Q}}
\def\bkN{{\rm I\kern-.17em N}}
\def\bkZ{{\rm I\kern-.17em Z}}
\def\bkC{\mathbb{C}}
%
%     index function
%
\def\uniset{{\rm 1\kern-.40em 1}}
%
%     =def
%
\newcommand{\eqdef}{\stackrel{\rm def}{=}}
%
%
%     Trace operator
%
%\DeclareMathOperator{\mtr}{Tr}
%
%
%  support
%\DeclareMathOperator{\msupp}{supp}
%
%     Standard array ({lcl}, with left brace)
%
\newenvironment{stdarray}{\[  \left\{ \begin{array}{lcl}}{\end{array} \right. \]}
\newcommand{\bstd}{\begin{stdarray}}
\newcommand{\estd}{\end{stdarray}}
%
%
%       numbered equation
%
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
%
%
\newcommand{\erps}{\varepsilon}
\newcommand{\tuntot}{t=1,\ldots,T}
\newcommand{\huntoh}{h=1,\ldots,H}
\newcommand{\untot}[1]{{#1}_1,\ldots,{#1}_T}
\newcommand{\thest}{\hat\theta_T}
\newcommand{\thesth}{\hat\theta^H_T}

% \DeclareMathOperator{\Co}{Co}
% \DeclareMathOperator{\mcov}{cov}
% \DeclareMathOperator{\plim}{plim}
% \DeclareMathOperator{\med}{median}

\newcommand{\hbn}{{\hat{\beta}_n}}
\newcommand{\htn}{{\hat{\theta}_n}}
\newcommand{\tzero}{{\theta_0}}
\newcommand{\bzero}{{\beta_0}}

\newcommand{\hxn}{{\hat{x}_n}}
\newcommand{\hyn}{{\hat{y}_n}}

\newcommand{\vv}{\vspace{1cm}}
%
%
% independence
\def\Perp{\perp\!\!\!\perp}

%
%   set
\newcommand{\set}[1]{\left\{#1\right\}}
%

% bold vectors
\let\vaccent=\v % rename built-in command \v{} as \vaccent{}
\renewcommand{\v}[1]{\mathbf{#1}} % for vectors
\newcommand{\gv}[1]{\boldsymbol{#1}} % for vectors of Greek letters
%

%
%        ABBREVS:
%
\newcommand{\rpo}{renegotiation-proof}
\newcommand{\rneg}{renegotiation}
\newcommand{\est}{estimation}
\newcommand{\iet}{int\'er\^et}
\newcommand{\dff}{dif\-f\'eren\-tiab}
\newcommand{\sm}{si\-mu\-la\-tion}
\newcommand{\mt}{m\'e\-tho\-de}
\newcommand{\dsq}{d\'e\-s\'e\-qui\-lib\-re}
\newcommand{\ler}{li\-n\'eaire}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
%
%
%       for referee reports
%
\newcommand{\pali}[2]{\item p.\ #1, l.\ #2 :}
\newcommand{\papar}[2]{\item p.\ #1, \P\  #2 :}
\newcommand{\padj}[1]{\item p.\ #1 :}
%
%
%        for SliTeX
%
\newcommand{\slili}[1]{\begin{slide}{} {\small #1} \end{slide}}
\newcommand{\veve}{\vspace{1cm}}
\newcommand{\lra}{$\longrightarrow$}
%
%
% independence
\def\Perp{\perp\!\!\!\perp}
%
%
%
%
%
%     journals
%
\newcommand{\ema}{{\it Econometrica~}}
\newcommand{\aer}{{\it American Economic Review~}}
\newcommand{\eer}{{\it European Economic Review~}}
\newcommand{\ann}{{\it Annales d'Economie et de Statistique~}}
\newcommand{\jet}{{\it Journal of Economic Theory~}}
\newcommand{\bje}{{\it Bell Journal of Economics~}}
\newcommand{\res}{{\it Review of Economic Studies~}}
\newcommand{\qje}{{\it Quarterly Journal of Economics~}}
\newcommand{\jap}{{\it Journal of Applied Econometrics~}}
\newcommand{\joe}{{\it Journal of Econometrics~}}
\newcommand{\jpe}{{\it Journal of Political Economy~}}
\newcommand{\jof}{{\it Journal of Finance~}}
%\newcommand{\ier}{{\it International Economic Review~}}
%
%    references
%

\newcommand{\adr}{Aghion-Dewatripont-Rey (1989)}
\newcommand{\badr}{{\bf Aghion, P., M. Dewatripont and P. Rey (1989)},
``Renegotiation Design with Unverifiable Information'', mimeo.}

\newcommand{\bouchia}{Bourguignon-Chiappori (1988)}
\newcommand{\bbouchia}{{\bf Bourguignon, F. and P.A. Chiappori (1988)}, ``An Econometric Model of the Inter\-nal La\-bour
Market'', \underline{Essays in Ho\-nour of Ed\-mond}
\underline{Malin\-vaud},
volume~3, MIT Press.}

\newcommand{\brasty}{Braverman-Stiglitz (1982)}
\newcommand{\bbrasty}{{\bf Braverman, A. and J. Stiglitz (1982)},
``Sharecropping and the Interlinking of Agrarian Markets'',  \aer,
 72, 695-715.}

\newcommand{\chiama}{Chiappori-Macho (1989)}
\newcommand{\bchiama}{{\bf Chiappori, P.A. and I. Macho (1989)},  ``Contrats de travail r\'ep\'{e}t\'{e}s~: le
r\^{o}le  de la m\'{e}moire'',\ann, 17, 47-70.}


\newcommand{\mathias}{Dewatripont (1988)}
\newcommand{\bmathias}{{\bf Dewatripont, M. (1988)}, ``Renegotiation
and Information Revelation Over Time  in Agency Contracts'', \res, 55, 377-390.}


\newcommand{\engran}{Engle-Granger~(1987)}
\newcommand{\bengran}{{\bf Engle, R.F. and  C. Granger (1987)},
``Cointegration and Error Correction: Representation, Estimation, and
Testing'',
\ema, 55, 251-276.}


\newcommand{\ehr}{Engle-Hendry-Richard~(1983)}
\newcommand{\behr}{{\bf Engle, R.F., D.F. Hendry and J.F. Richard
(1983)}, ``Exogeneity'', \ema, 44, 305-321.}


\newcommand{\futi}{Fudenberg-Tirole (1990)}
\newcommand{\bfuti}{{\bf Fudenberg, D. and J. Tirole (1990)}, ``Moral
Hazard and Renegotiation in Agency Contracts'',  \eca, 58, 1279-1319.}

\newcommand{\gmtpml}{Gouri\'eroux-Mon\-fort-Trog\-non~(1984)}
\newcommand{\bgmtpml}{{\bf Gouri\'eroux, C., A. Monfort and A. Trognon~(1984)},  ``Pseudo-Maximum Likelihood Methods: Theory'',
 \ema, 52, 681-700.}

\newcommand{\gmtcorrel}{Gouri\'eroux-Monfort-Trognon~(1985)}
\newcommand{\bgmtcorrel}{{\bf Gouri\'eroux, C., A. Monfort and A.
Trognon (1985)}, ``A General  Approach to Serial Correlation'', {\it
Econometric Theory}, 1, 315-340.}

 \newcommand{\greela}{Green-Laffont (1988)}
\newcommand{\bgreela}{{\bf Green, J. and J.J. Laffont (1988)},
``Contract Renegotiation and the Underinvestment Effect'',  Harvard Institute of Economic Research Discussion Paper \#
1385.}

\newcommand{\hk}{Hart-Kreps (1986)}
\newcommand{\bhk}{{\bf Hart, O. and  D. Kreps (1986)},
``Price-Destabilizing Speculation'', \jpe, 94, 927-952.}

\newcommand{\hamoo}{Hart-Moore (1988)}
\newcommand{\bhamoo}{{\bf Hart, O. and J. Moore (1988)},  ``Incomplete Contracts and Renegotiation'', \eca, 55,
303-328.}

\newcommand{\hati}{Hart-Tirole (1988)}
\newcommand{\bhati}{{\bf Hart, O. and J. Tirole (1988)}, ``Contract
Renegotiation and Coasian Dynamics'', \res, 55,  509-540.}

\newcommand{\hmlinear}{Holmstrom-Milgrom (1987)}
\newcommand{\bhmlinear}{{\bf Holmstrom, B. and  P. Milgrom (1987)}, ``Aggregation and Linearity in the Provision of
Intertemporal Incentives'', \eca,
55, 303-328.}

\newcommand{\johan}{Johansen~(1988)}
\newcommand{\bjohan}{{\bf Johansen, S. (1988)}, ``Statistical Analysis
of Cointegration Vectors'', {\it Journal of Economic Dynamics and
Control}, 12, 231-254.}


\newcommand{\lati}{Laffont-Tirole (1991)}
\newcommand{\blati}{{\bf Laffont, J.J. and J. Tirole (1991)}, ``Adverse
Selection and Renegotiation in Procurement'', \res, 57, 597-625.}

\newcommand{\lamb}{Lambert (1983)}
\newcommand{\blamb}{{\bf Lambert, R. (1983)}, ``Long-term Contracts and
                        Moral Hazard'', \bje, 14, 441-452.}


\newcommand{\lsun}{Laroque-Salani\'e~(1989)}
\newcommand{\blsun}{{\bf Laroque, G. and B. Salani\'e~(1989)}, ``Estimation of Multimarket Fix-Price Models:
An Application of Pseudo-Maximum Likelihood Methods'', \ema, 57,
831-860.}

\newcommand{\lsdeux}{Laroque-Salani\'e~(1994)}
\newcommand{\blsdeux}{{\bf Laroque, G. and B. Salani\'e~(1994)},
``Estimating the Canonical Disequilibrium Model:
Asymptotic Theory and Finite-Sample Properties'', \joe, 62, 165-210.}

\newcommand{\lstrois}{Laroque-Salani\'e~(1993)}
\newcommand{\blstrois}{{\bf Laroque, G. and B. Salani\'e~(1993)},
``Simulation-based Estimation of Models with
Lagged Latent Variables'', \jap, 8, S119-S133.}


\newcommand{\lerman}{Lerman-Manski~(1981)}
\newcommand{\blerman}{{\bf Lerman, S. and C.F. Manski~(1981)},
``On the Use of Simulated Frequencies to Approximate Choice
Probabilities'', in {\it Structural Analysis of Discrete Data with
Economic Applications}, C.F. Manski and D. McFadden eds, Cambridge:
MIT Press.}

\newcommand{\malspin}{Malcomson-Spinnewyn (1988)}
\newcommand{\bmalspin}{{\bf Malcomson, J. and F. Spinnewyn (1988)},  ``The Multipe\-riod Prin\-cipal-Agent Problem'', \res, 55, 391-408.}


\newcommand{\mamoo}{Maskin-Moore (1988)}
\newcommand{\bmamoo}{{\bf Maskin, E. and J. Moore (1988)}, ``Implementation and Renegotiation'', mimeo.}


\newcommand{\mcfa}{McFadden~(1989)}
\newcommand{\bmcfa}{{\bf McFadden, D.~(1989)},  ``A Method of Simulated
Moments for Estimation of
Discrete Response Models Without Numerical Integration'', \ema, 57,
995-1026.}


\newcommand{\newb}{Newbery (1987)}
\newcommand{\bnewb}{{\bf Newbery, D. (1987)}, ``When Do Futures
Destabilize Spot Prices?'', \ier, 28,
 291-297.}


\newcommand{\newest}{Newey-West~(1987)}
\newcommand{\bnewest}{{\bf Newey, W. and K. West (1987)} ``A Simple, Positive,
Semi-defi\-nite, Hetero\-ske\-das\-ticity and Auto\-corre\-lation
Con\-sis\-tent Cova\-riance Mat\-rix'', {\it Econometrica}, 55,
703-708.}

\newcommand{\pakes}{Pakes~(1986)}
\newcommand{\bpkes}{{\bf Pakes, A.~(1986)},  ``Patents as Options: Some
Estimates of the  Value of
Holding European Patent Stocks'', \ema, 54, 755-785.}

\newcommand{\pkpo}{Pakes-Pollard~(1989)}
\newcommand{\bpkpo}{{\bf Pakes, A. and D. Pollard~(1989)},
``Simulation and the Asymptotics of Optimization
Estimators'', \ema, 57, 1027-1057.}


\newcommand{\park}{Park~(1992)}
\newcommand{\bpark}{{\bf Park, J.Y. (1992)}, ``Canonical Cointegration
Regressions'', \ema, 60, 119-143.}


\newcommand{\quro}{Quandt-Rosen~(1986)}
\newcommand{\bquro}{{\bf Quandt, R. and H. Rosen (1986)},
``Unemployment, Disequilibrium and the Short-run Phillips Curve: An
Econometric Approach'', \jap, 1, 235-253.}


\newcommand{\qurobk}{Quandt-Rosen~(1988)}
\newcommand{\bqurobk}{{\bf Quandt, R. and H. Rosen (1988)},
{\it The Conflict Between Equilibrium and Disequilibrium Theories: The
Case of the US Labor Market}, Upjohn Institute.}

\newcommand{\rey}{Rey (1988)}
\newcommand{\brey}{{\bf Rey, P. (1988)}, ``A Note on the Result of
\roger\ on the  Desirability of Constrained Savings'', mimeo.}

\newcommand{\rsun}{Rey-Salani\'{e} (1990)}
\newcommand{\brsun}{{\bf Rey, P. and B. Salani\'{e} (1990)},
``Long-term, Short-term and Renegotiation : On the
Value of Commitment in Contracting'',
                         \eca, 58, 597-619.}

\newcommand{\rsdeux}{Rey-Salani\'{e} (1991)}
\newcommand{\brsdeux}{{\bf Rey, P. and B. Salani\'{e} (1991)}, ``The Value of
Commitment in Contracting with Asymmetric Information'', mim\'eo.}


\newcommand{\richa}{Richard~(1992)}
\newcommand{\bricha}{{\bf Richard, J.F. (1992)}, ``Dynamic Latent
Variable Models---Likelihood Evaluation'', mimeo.}

\newcommand{\roger}{Rogerson (1985)}
\newcommand{\broger}{{\bf Rogerson, W. (1985)}, ``Repeated
                Moral Hazard'', \eca, 53, 69-76.}


\newcommand{\rosti}{Rothschild-Stiglitz~(1976)}
\newcommand{\brosti}{{\bf Rothschild, M. and J. Stiglitz~(1976)}, ``Equilibrium in
Competitive Insurance Markets: An Essay on the Economics of Imperfect
Information'', {\it Quarterly Journal of Economics}, 90, 629-650.}


\newcommand{\sal}{Salani\'e~(1991)}
\newcommand{\bsal}{{\bf Salani\'e, B.~(1991)}, ``Wage and Price
Adjustment in a Multimarket
Disequilibrium Model'', \jap, 6, 1-15.}

\newcommand{\shav}{Shavell (1976)}
\newcommand{\bshav}{{\bf Shavell, S. (1976)},``On Moral Hazard and Insurance'', Harvard Institute
of      Economic Research Discussion Paper \# 494.}


\newcommand{\stein}{Stein (1987)}
\newcommand{\bstein}{{\bf Stein, J. (1987)}, ``Informational
Externalities and Welfare-Reducing
 Speculation'', \jpe, 95, 1123-1145.}

%















